Quantization of gauge fields, graph polynomials and graph cohomology

We review quantization of gauge fields using algebraic properties of 3-regular graphs. We derive the Feynman integrand at n loops for a non-abelian gauge theory quantized in a covariant gauge from scalar integrands for connected 3-regular graphs, obtained from the two Symanzik polynomials. The transition to the full gauge theory amplitude is obtained by the use of a third, new, graph polynomial, the corolla polynomial. This implies effectively a covariant quantization without ghosts, where all the relevant signs of the ghost sector are incorporated in a double complex furnished by the corolla polynomial -we call it cycle homology- and by graph homology.

==> graphs1.tex <==
% graphs.t1 -- generated from graphs.mp
\fmfL(0.246,-1.5676,rt){$2$}%
\fmfL(0.246,16.5676,rb){$1$}%
\fmfL(14.754,-1.5676,lt){$3$}%
\fmfL(14.754,16.5676,lb){$4$}%


==> graphs128.tex <==
% graphs.t128 -- generated from graphs.mp
\fmfL(20,22.00752,b){$3$}%
\fmfL(20,-2.0075,t){$4$}%
\fmfL(40.00002,7.9925,t){$5$}%
\fmfL(60,22.0075,b){$6$}%
\fmfL(60,-2.0075,t){$7$}%
\fmfL(-2.0075,10,r){$1$}%
\fmfL(82.0075,10,l){$2$}%
\fmfL(12.0075,10,l){a}%
\fmfL(27.9925,10.00002,r){b}%
\fmfL(52.0075,10,l){c}%
\fmfL(67.9925,10,r){d}%


==> graphs129.tex <==
% graphs.t129 -- generated from graphs.mp
\fmfL(19.99997,22.00746,b){$3$}%
\fmfL(19.99995,-2.00749,t){$4$}%
\fmfL(12.00749,9.99998,l){a}%
\fmfL(27.99243,9.99998,r){b}%


==> graphs130.tex <==
% graphs.t130 -- generated from graphs.mp
\fmfL(19.99997,22.00746,b){$6$}%
\fmfL(19.99995,-2.00749,t){$7$}%
\fmfL(12.00749,9.99998,l){c}%
\fmfL(27.99243,9.99998,r){d}%


==> graphs171.tex <==
% graphs.t171 -- generated from graphs.mp
\fmfL(15.00002,11.98872,t){\scriptsize $5$}%
\fmfL(2.37314,-0.7838,rt){\scriptsize $2$}%
\fmfL(2.37314,30.7838,rb){\scriptsize $1$}%
\fmfL(27.62686,-0.7838,lt){\scriptsize $3$}%
\fmfL(27.62686,30.7838,lb){\scriptsize $4$}%
\fmfL(3.98886,15,r){\scriptsize $v$}%
\fmfL(26.01112,14.99998,l){\scriptsize $w$}%


==> graphs172.tex <==
% graphs.t172 -- generated from graphs.mp
\fmfL(14.99998,-3.01125,t){\scriptsize $3$}%
\fmfL(14.99998,18.01123,b){\scriptsize $4$}%
\fmfL(-1.00375,7.50002,r){\scriptsize $1$}%
\fmfL(31.00375,7.50002,l){\scriptsize $2$}%
\fmfL(12.51875,7.49998,r){\scriptsize $v$}%
\fmfL(16.47745,7.49998,l){\scriptsize $w$}%


==> graphs173.tex <==
% graphs.t173 -- generated from graphs.mp
\fmfL(17.50006,19.50757,b){$1$}%
\fmfL(17.50008,-2.00749,t){$2$}%
\fmfL(-2.0075,8.75002,r){$3$}%
\fmfL(37.0075,8.75002,l){$4$}%
\fmfL(10.75754,8.75003,l){a}%
\fmfL(24.24258,8.75006,r){b}%


==> graphs2.tex <==
% graphs.t2 -- generated from graphs.mp
\fmfL(7.50002,3.48499,t){$e$}%
\fmfL(0.246,-1.5676,rt){$2$}%
\fmfL(0.246,16.5676,rb){$1$}%
\fmfL(14.754,-1.5676,lt){$3$}%
\fmfL(14.754,16.5676,lb){$4$}%


==> graphs59.tex <==
% graphs.t59 -- generated from graphs.mp
\fmfL(11.50941,18.49055,rb){$3$}%
\fmfL(11.50941,1.50941,rt){$4$}%
\fmfL(17.99246,9.99998,r){$5$}%
\fmfL(28.49054,18.49054,lb){$6$}%
\fmfL(28.49054,1.50943,lt){$7$}%
\fmfL(-2.0075,10,r){$1$}%
\fmfL(42.0075,10,l){$2$}%


==> graphs8.tex <==
% graphs.t8 -- generated from graphs.mp
\fmfL(-1.56624,7.52173,rt){\scriptsize $1$}%
\fmfL(4.93588,7.14484,r){\scriptsize $2$}%
\fmfL(15.06438,7.14478,l){\scriptsize $3$}%
\fmfL(21.56659,7.52156,lt){\scriptsize $4$}%
\fmfL(10,-2.0075,t){\scriptsize $v$}%

